Fast modeling of regenerative amplifier free-electron lasers

High-gain free-electron lasers (FELs) are becoming important light sources at short wavelengths such as the EUV and X-ray regimes. A particularly promising concept is the regenerative amplifier FEL (RAFEL), which can greatly increase the brightness and stability of a single pass device. One of the critical challenges of the x-ray RAFEL is maintaining electron-optical overlap over the relatively large (hundreds of meters) footprint of the system. Numerical modeling of x-ray RAFELs with angular and positional errors is critical for designing stable cavities, as well as to predict signatures of specific misalignment effects. Full-scale simulations of x-ray FELs are incredibly time-consuming, making large-scale parameter searches intractable on reasonable timescales. In this paper, we present a semi-analytical model that allows to investigate realistic scenarios - x-ray cavity without gain ("cold cavity" or x-ray FEL oscillator) and x-ray RAFEL - in the presence of angular/positional errors and electron trajectory oscillation. We especially focus on fast modeling of the FEL process and x-ray optics, while capturing effects pertaining to actual experimental setups at the Linac Coherent Light Source (LCLS) at SLAC. Such a method can be used to explore RAFEL at other wavelengths by suitable replacement of the optics modeling.

==> new_intro_draft.tex <==
Free-electron lasers (FELs) have revolutionized the scope of light-driven science. FELs are high-power, ultra-fast radiation sources which work by wiggling a relativistic electron beam inside of a magnetic undulator prompting the beam to emit synchrotron radiation. The central frequency of an FEL is tunable across the entire electromagnetic spectrum simply by changing the electron beam energy or the undulator field strength or period, allowing them to fill critical gaps left by conventional laser technology -- most notably in the THz, EUV, and x-ray spectral ranges. The earliest FELs operated at relatively long wavelengths, in the infrared and optical regimes \cite{hogan1998measurements,hogan1998measurements2,milton2000observation,milton2001exponential}. Those early FELs looked in concept very much like a traditional laser: a gain medium (the FEL) was enclosed within an optical cavity capable of storing the output radiation so that it could be amplified further and further with fresh electron beams \cite{madey1971stimulated,deacon1977first,nguyen1999first}. Similarly to conventional lasers, FELs of this form could be operated in a low gain-per-pass configuration (termed FEL osillator or FELO), or in a high gain-per-pass configuration (termed regenerative amplifier FEL or RAFEL). 

The true power of the FEL lies in its tunability, so the natural question is how to extend it to photon energies that are inaccessible by conventional laser technologies: x-rays and beyond \cite{murphy1985free,tatchyn1996research,pellegrini19932}. In this regime difficulties arise due to the lack (at the time) of high reflectivity, large angle mirrors to form the optical cavity. As a result, the x-ray FEL (XFEL) has in every realization to date been a single-pass device, where the radiation is instantiated either by seeding with an external laser (only for very soft x-rays) or by amplifying the spontaneous radiation emitted by the electron beam due to its shot noise -- the latter is called self-amplified spontaneous emission (SASE). SASE XFELs have been tremendously successful -- they are almost completely transversely coherent, but they suffer from a lack of temporal coherence  and shot-to-shot stability arising from the random nature of the startup. These issues limit the peak spectral brightness that can be obtained from SASE XFELs. Many concepts have been proposed to improve the temporal coherence, but for hard x-rays all are inherently limited by the fact that the start-up is always random. 

The discovery of very high ($\sim 99$\%) reflectivity Bragg reflections of hard x-rays from crystal structures \cite{liss2000storage,shvyd2003x,shvyd2011near} revitalized the discussions around cavity-based FELs in the x-ray regime \cite{huang2006fully,kim2008proposal}. An XFEL enclosed by a Bragg crystal cavity, which would provide both spectral and angular filtering to the radiation, promises to deliver fully coherent, high power, stable x-ray pulses. As with the earliest FELs, cavity-based x-ray FELs (CBXFELs) are envisioned in two different regimes: the XFEL oscillator (XFELO) and the x-ray regenerative amplifier FEL (XRAFEL). There are several ongoing projects aimed at the first experimental demonstration of the CBXFEL concept at LCLS (USA) \cite{marcus2019cavity}, EuXFEL (Germany) \cite{ PhysRevAccelBeams.26.020701} and SHINE (China) \cite{Huang2023} facilities. One of the key difficulties associated with the demonstration of CBXFELs is proper alignment of the optical cavity -- the XFEL gain medium has a 10s to 100 meter scale footprint while Bragg reflections have typical angular acceptances on the scale of 10 $\mu$rad. Thus these optical cavities must be aligned in principle with sub-$\mu$rad precision, and critically the effects of and tolerance to misalignment must be well understood.

In order to fully understand the tolerances and optimal design strategies for CBXFELs, accurate numerical modeling is essential. This is true at any wavelength, from the original IR cavity-based FELs, to extreme ultraviolet cavity-based FELs for lithography, to the x-ray regime. Cavity-based FELs pose a unique modeling challenge -- single-pass FEL simulations are notoriously time consuming and they must now be combined with Fourier optics propagation of the resulting fields through long cavities, and then all of this must be done over the tens to hundreds of passes required for the system to reach a steady state. In the low gain, FELO case, these challenges are alleviated by the fact that the impact of the FEL on the transverse dynamics of the photons is weak and the dynamics are dominated by the optical cavity. For RAFELs this is no longer the case, as high-gain FELs exhibit strong optical guiding effects -- both gain guiding and refractive guiding -- which play a dominant role in the dynamics of the optical pulse in the cavity. Thus, accurate modeling of RAFELs mandates accurate modeling of the FEL interaction, which makes simulations extremely time-consuming. This limits the extent to which the full RAFEL parameter space can be explored, holding back any individual project, and the field as a whole. Unfortunately, there is no real getting around how time consuming full fidelity RAFEL simulations are, however there is a space for faster models with more restricted accuracy which can be used to perform wide, coarse scans of the parameter space and study misalignment tolerances. The results found by such fast models could be then be used as starting points for finer scans with higher fidelity simulations.

In this paper we present a fast, semi-analytical model for RAFEL dynamics tailored precisely to that purpose. We base our technique on a time-independent, high-gain FEL gain guiding model combined with gaussian beam propagation. We start from the general 3D FEL equations which are applicable at any wavelength, but in our discussions we will focus on parameters relevant to hard XRAFEL systems. 

It is worth taking a moment to discuss the approximations behind the model. These approximations are all motivated by the typical critical features of a  RAFEL system. Although the transverse FEL radiation mode is not exactly gaussian, it is highly transversely coherent and can be modeled as gaussian for the sake of simplicity and speed. Furthermore, our model is strictly valid only in the linear regime of the FEL before power saturation. This choice is made first and foremost because it enables fast semi-analytic methods. It is also in line with common RAFEL design methodologies which avoid allowing the FEL to go deep into saturation in a single pass. There are several reasons for that methodology. At saturation the transverse mode quality suffers \cite{saldin2003coherence,saldin2010statistical,geloni2010coherence} and the side-band instability causes the emission of unwanted frequency components \cite{kroll1981free,marcus2017x}. Furthermore, deep in saturation the refractive and gain guiding responsible for the high transverse mode quality significantly reduces \cite{huang2002transverse}. As we will find in our numerical examples later in the paper, for a well-designed RAFEL the linear theory is sufficient for finding good working points which can be further refined with traditional simulation tools. Conveniently, in the linear regime the FEL acts as a linear amplifier and does not couple different frequency components together. As a result, single frequency (or time-independent) modeling is sufficient to capture the essential physics. 

The paper is organized as follows. We first introduce gaussian beam parameterization and discuss the high-gain, time-independent FEL model. 
We then provide several concrete examples of where our technique can be applied, and use it for the case of an x-ray cavity with no gain (cold cavity), and a high-gain XFEL amplifier with and without e-beam trajectory oscillations. Finally, we utilize the unique capabilities of a fast modeling scheme to optimize the focusing system for an XRAFEL, and to understand the tolerance of a given XRAFEL design to increasingly large angular errors.




==> original_intro.tex <==
X-ray free-electron lasers (XFELs) have revolutionized scientific research by offering unprecedented capabilities for x-ray imaging of complex physical systems. They are crucial in advancing our understanding of the femtosecond-angstrom (fs-A) scale and have far-reaching implications in the fields of biology, chemistry, materials science, and physics. Today, single pass self-amplified spontaneous emission (SASE) FELs are the workhorse of ultrafast, high intensity x-ray science. While SASE FELs have been tremendously successful, they suffer from a lack of temporal coherence and shot-to-shot stability. 
To further improve spectral coherence, brightness, and stability, one can consider encasing an XFEL in an optical cavity, similar to a conventional laser \cite{huang2006fully, kim2008proposal}. In this regime, the x-ray radiation is recirculated and interacts with the e-beam multiple times, reaching properties beyond what a single pass, high-gain system can provide. These systems are commonly known as cavity-based XFELs (CBXFELs). A simple schematic of an example CBXFEL geometry is shown in Figure~\ref{fig:cartoon}.

\begin{figure}[b]
    \centering
    \includegraphics{Fig1.pdf}
    \caption{A possible example CBXFEL geometry. A rectangular cavity formed by four Bragg reflecting crystals wraps an undulator of length $L_u$. On either side of the cavity there are focusing lenses with focal length $f$. The mirror immediately following the undulator is labeled $M_1$.}
    \label{fig:cartoon}
\end{figure}

Notably, there are several ongoing projects aimed at the first experimental demonstration of this concept at LCLS (USA) \cite{marcus2019cavity}, EuXFEL (Germany) \cite{ PhysRevAccelBeams.26.020701} and SHINE (China) \cite{Huang2023} facilities. 
CBXFELs can be classified by high- and low-gain cases. In the high-gain case (single-pass power gain of about 50 and larger), the system behaves similarly to a conventional regenerative amplifier, in which the saturation is achieved in a relatively small number of cavity passes \cite{marcus2020refractive}. In the low gain case (single-pass power gain less than 5), the system behaves like a laser oscillator, gradually building up a coherent cavity pulse from noise in many (several hundred) passes \cite{Qin:2018xer}. For low gain CBXFELs, the transverse dynamics and stability of the system are dominated by the optical elements \cite{PhysRevAccelBeams.25.090702}. For high gain CBXFELs this is not the case, as high gain FELs exhibit optical guiding properties that are able to both steer and focus the radiation pulse \cite{scharlemann1985optical}. This paper focuses on the high-gain case, which we will later refer to as x-ray regenerative amplifier FEL or XRAFEL.
Furthermore, we point out that all CBXFELs are currently envisioned in the hard x-ray regime, where one can use highly reflective Bragg crystals as cavity mirrors. In the soft x-ray regime, due to the lack of efficient optics, this concept remains to be explored. We also note that XRAFEL operating in the EUV regime can be considered an alternative for EUV lithography \cite{10.1117/1.JMM.11.2.021122, 10.1117/12.2085538}.  

To investigate CBXFEL operation, one has to perform FEL simulations for each cavity pass in addition to tracking the radiation through the optical cavity elements. The number of simulated passes can be quite large when considering cavity outcoupling before the cavity operates in a steady-state regime. A time-dependent 3D study of the XRAFEL parameter space can quickly become very time-consuming in this case \cite{Qin:2018xer, marcus2020refractive, PhysRevSTAB.10.030702, Freund_2019}. However, very often, for the initial design and alignment studies, full-scale numerical simulations are not required. Instead, one would prefer a quick simulation tool that captures only the most important cavity physics, allowing a quick sweep through the parameter space, leaving the traditional methods to be used for validation and further refinement. 

Our paper presents a fast semi-analytical method tailored to this purpose. We base our technique on a time-independent, high-gain FEL gain-guiding model combined with gaussian beam propagation. It is worth taking a moment to discuss the approximations behind the model. These approximations are all motivated by the typical critical features of an XRAFEL system. Although the transverse FEL radiation mode is not exactly gaussian, it is highly transversely coherent and can be modeled as gaussian for the sake of simplicity and speed. Furthermore, our model is strictly valid only in the linear regime of the FEL before power saturation. This choice is made first and foremost because it enables fast semi-analytic methods. It is also in line with common XRAFEL design methodologies which avoid allowing the FEL to go deep into saturation in a single pass. There are several reasons for that methodology. At saturation the transverse mode quality suffers \cite{saldin2003coherence,saldin2010statistical,geloni2010coherence} and the side-band instability causes the emission of unwanted frequency components \cite{kroll1981free,marcus2017x}. Furthermore, deep in saturation the refractive and gain guiding responsible for the high transverse mode quality significantly reduces \cite{huang2002transverse}. As we will find in our numerical examples later in the paper, for a well-designed XRAFEL the linear theory does a sufficiently good job of finding good working points which can be further refined with traditional simulation tools. Conveniently, in the linear regime the FEL acts as a linear amplifier and does not coupled different frequency components together. As a result, single frequency (or time-independent) modeling is sufficient to capture the essential physics. 

The paper is organized as follows. We first introduce gaussian beam parameterization and discuss the high-gain, time-independent FEL model. 
We then provide several concrete examples of where our technique can be applied, and use it for the case of an x-ray cavity with no gain (cold cavity), and a high-gain XFEL amplifier with and without e-beam trajectory oscillations. Finally, we utilize the unique capabilities of a fast modeling scheme to optimize the focusing system for an XRAFEL, and to understand the tolerance of a given XRAFEL design to increasingly large angular errors.
